The Evolution of central and satellite galaxies in the local universe: Insights from galactic archeology

This thesis investigates the evolution of galaxies in diverse environments, utilizing Sloan Digital Sky Survey (SDSS) data to explore the impact of environmental richness on central and satellite galaxies across stellar mass ranges, compared to isolated systems. The sample is limited to 0.03 < z < 0.1 and apparent magnitudes brighter than 17.78, ensuring spectroscopic completeness and reliable stellar population estimates. Galaxies are categorized by environment as field or cluster/group systems, with further separation into satellites and centrals. By analyzing the star formation rate (SFR)-stellar mass plane, this work identifies systematic differences in the blue cloud (BC), green valley (GV), and red sequence (RS) across environments. Morphological and stellar population analyses reveal that T-type, metallicity, and stellar age transitions highlight the role of environmental quenching. A newly introduced T-Type \emph{vs.} specific SFR diagram provides evidence that morphological transformation precedes full quenching. Correlating galaxy properties with time since infall through projected phase space confirms the delayed-then-rapid quenching model for low- and intermediate-mass galaxies, extending it to morphology. Time-scales for quenching and morphological transitions are also derived as a function of stellar mass.

==> folha-de-aprova____o.tex <==
\begin{center}

Vitor Medeiros Sampaio

\vspace{1.0cm}

The Evolution of central and satellite galaxies
in the local universe: Insights from galactic
archeology

\vspace{1.0cm}

\begin{flushright}
\begin{minipage}{1.0\textwidth}

{Tese apresentada ao Programa de Pós-graduação em Astrofísica e Física Computacional da Universidade Cidade de São Paulo, como requisito parcial para obtenção do título de Doutor, sob a orientação do Dr. Reinaldo Ramos de Carvalho}

\end{minipage}
\end{flushright}

\vfill

\begin{flushleft}

Aprovada em XXXXX

\end{flushleft}

\vfill

BANCA EXAMINADORA

\vfill

\hrulefill \\Prof. Dr. Reinaldo Ramos de Carvalho - Orientador\\Universidade Cidade de São Paulo\\

\vfill

\hrulefill \\Prof. Dr. \\University of Nottingham\\

\vfill

\hrulefill \\Prof. Dr. \\Universidade Cidade de São Paulo\\

\vfill

\hrulefill \\Prof. Dr. \\Universidade Tecnológica Federal do Paraná\\

\vfill

\hrulefill \\Prof. Dr. \\EACH - Universidade de São Paulo\\

\vfill

\end{center}

\newpage

